Enclave-Aware Compartmentalization and Secure Sharing with Sirius

Hardware-assisted trusted execution environments (TEEs) are critical building blocks of many modern applications. However, they have a one-way isolation model that introduces a semantic gap between a TEE and its outside world. This lack of information causes an ever-increasing set of attacks on TEE-enabled applications that exploit various insecure interactions with the host OSs, applications, or other enclaves. We introduce Sirius, the first compartmentalization framework that achieves strong isolation and secure sharing in TEE-assisted applications by controlling the dataflows within primary kernel objects (e.g. threads, processes, address spaces, files, sockets, pipes) in both the secure and normal worlds. Sirius replaces ad-hoc interactions in current TEE systems with a principled approach that adds strong inter- and intra-address space isolation and effectively eliminates a wide range of attacks. We evaluate Sirius on ARM platforms and find that it is lightweight ($\approx 15K$ LoC) and only adds $\approx 10.8\%$ overhead to enable TEE support on applications such as httpd, and improves the performance of existing TEE-enabled applications such as the Darknet ML framework and ARM's LibDDSSec by $0.05\%-5.6\%$.

==> ack.tex <==
\section{Acknowledgment}

==> apps.tex <==
\begin{figure*}
\begin{subfigure}{.30\textwidth}
\centering
\includegraphics[height=3.2cm]{images/httpd.pdf}%
\caption{Apache httpd}\label{fig:httpd}
\end{subfigure}\hfill
\begin{subfigure}{.28\textwidth}
\centering
\includegraphics[height=3.2cm]{images/ml.pdf}%
\caption{Darknet ML framework}\label{fig:darknet}
\end{subfigure}\hfill
\begin{subfigure}{.28\textwidth}
\centering
\includegraphics[width=6cm, height=3.2cm]{images/dds.pdf}%
\caption{DDS-based applications}\label{fig:dds}
\end{subfigure}
\caption{High-level architecture of Sirius-protected applications}
  \label{fig:arch}
\end{figure*}


==> cve-tab.tex <==
\begin{table}[t]
    \hline
\resizebox{\columnwidth}{!}{%
  \footnotesize
  \begin{tabular}{|c|l|l|c|}
    & \bf Threat       & \bf Description  & \bf Sirius \\
    \hline
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\bf General threats }}}
        & \cve{2017-0597} &  Privilege gain     & \chk \\ 

    & \cve{2019-2023} & Android permissions bypass &\chk \\
  & \cve{2019-5736} & Container escape  &\chk \\
    & \cve{2019-10063} & Sandbox bypass     & \chk \\
    & \cve{2019-16884} & SELinux/AppArmor bypass       & \chk \\
    & \cve{2019-14287} &  Achieve root   &  \chk\\
    & \cve{2018-18955} & Namespace bypass   & \chk \\
    
    & \cve{2018-9488} & Permissions bypass      & \chk \\
       & \cve{2017-13236} & Keystore permissions bypass      & \chk \\
 

    \hline
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\bf In-Process threats}}}
    
    & \cve{2019-9345} & Shared mapping bug  &\chk \\
    & \cve{2019-9423} & missing bounds check      & \chk \\
    & \cve{2019-15295} & unsafe third party library      & \chk \\
    & \cve{2019-1278} &  unsafe third party library   &  \chk\\
    & \cve{2018-0487} & unsafe third party library    & \chk \\
    
    & \cve{2017-1000376} &  unsafe native bindings     & \chk \\

    & \cve{2014-0160} &  Heartbleed bug     & \chk \\ 
  
    \hline
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\bf Other}}}

    

    & \cve{2018-0497} & SW side-channels  &   \\
      & \cve{2017-5754} & HW side-channels & \\
    \hline
    

  \end{tabular}}
  \caption{A representative selection of vulnerabilities that cause sensitive content leakage. The attacks with a tick can be mitigated by using {\bf Sirius}.}
  \label{cvetab}
\end{table}





==> hw-assum.tex <==
\subsection{Hardware assumptions}\label{memdomain}

Recent CPUs have supported various ways of efficient memory protection and systems isolations~\cite{arm2012architecture,mpk}.
This paper primarily describes the design of Sirius on ARMv7-A.

\textbf{Memory management:}
Sirius, in particular, relies on the underlying hardware features for fine- and coarse-grained intra-process memory isolation.
The ARMv7 memory management unit (MMU) consists of a TLB that caches entries. These consist of a virtual base address, a physical base address, Address Space Identifier (ASID) tags, and a set of flags for access control and other page attributes.
It supports a two-level hierarchical page table when using a short-descriptor translation table format, and supports variable page sizes (1GB, 1MB, 64KB, and 4KB).

ARM supports two page tables simultaneously, using the hardware registers TTBR0 and TTBR1. A virtual address is mapped to a physical address by the CPU, depending on settings in TTBRC. This control register has a field that sets a split point in the address space; addresses below the cutoff value are mapped through the page tables pointed to by TTBR0 (used per process), and addresses above the cutoff value are mapped through TTBR1 (used by the kernel). 

Since the introduction of ARMv5, the translation tables hold access permission fields and a \textbf{domain field}. ARM memory domains are a lesser-known memory access control mechanism independent of the widely used paging mechanism. Each page table entry has 4 bits allocated to hold a domain ID ranging from $D0$ to $D15$. Access control for each domain is handled by setting a domain access control register (DACR) in $CP15$, which is a 32-bit register only accessible in the privileged processor modes. Each domain is assigned two bits in DACR, which defines its access rights. 

\input{domains.tex}

The four possible access rights for a domain are No Access, Manager, Client, and Reserved (see Table~\ref{domains}).  Those fields let the processor ~\rom{1} prohibit access to the domain mapped memory--No Access;~\rom{2} allow unlimited access to the memory despite permission bits in the page table-- Manager; or~\rom{3} let the access right be the same as the page table permissions--Client. Any access violation causes a domain fault, and changes to the DACR are low cost and activated without affecting the TLB. 

ARM memory domains look like a good building block for in-process memory protection.  Changing domain permissions does not require TLB flushes, and they do not require extensive modifications to the kernel memory management structures that might otherwise introduce security holes due to inevitable TLB and memory management bugs~\cite{tlbbug}.
However, the current hardware implementation,~\num{1}only apply to first-level entries,~\num{2}relies on a 32-bit DACR register and so supports only up to 16 domains,~\num{3} requires syscall for changing the DACR that is a fast but privileged operation,~\num{4}do not allow directly marking a domain as read-only, write-only, or exec-only, that make it suitable for efficient but more coarse-grained isolation.

Hence the Sirius kernel provides a unifying abstraction for unlimited intra-process isolated units of memory (we call it \textmu Tiles), which backed with MMU or ARM-MD features to show the abstraction extendability as well as the effect of these hardware features on the right balance between efficiency and isolation granularity. 

\textbf{Security extensions:} or TrustZone\cite{tzman} is a System-On-Chip (SoC) security mechanism introduced with ARMv6 in most ARM Cortex-A and Cortex-M processors. 
The TrustZone hardware architecture can be seen as a dual-virtual system that allows partitioning of all system’s hardware resources, including the processor, memory, and peripherals into two execution environments. The resource partitioning to secure and non-secure(S/NS) can be done using Trustzone AXI components. For example, TrustZone Address Space Controller (TZASC) partitions a single AXI slave such as an off-SoC DRAM, while TrustZone Memory Adapter (TZMA) is used for partitioning on-SoC memory such SRAM. TrustZone Protection Controller (TZPC) signal configures peripherals. The Generic Interrupt Controller (GIC) supports both Secure and Non-secure prioritized interrupt sources. Both worlds have their own user space and kernel space (and even the hyp mode from ARMV8). The two worlds can communicate with each other under the strict supervision of a Secure Monitor running in monitor mode (EL3) via a Secure Monitor Call (SMC) instruction. 


We now describe the implementation of \textmu Tiles, which aims to provide practical intra-process isolation through a higher-level interface that hides the difficulties described earlier (\S\ref{challenges}) in utilizing hardware protection primitives.

\textbf{Design Principles}\\

The \textmu Tiles interface aims to enforce least privilege principle for memory accesses via the following guidelines:
\textbf{Fine-grained trust:}  All threads of execution should be able to define their security policies and trust models to selectively protect their sensitive resources. Current OS security models of sharing (``everything-or-nothing'') are not flexible enough for defining fine-grained trust boundaries within processes or threads (lightweight processes).\\
\textbf{Compatibility:} It is difficult to provide strong security guarantees with no code modifications, and \textmu Tiles is no exception. We move most of these modifications into the Linux kernel (increasingly popular for embedded deployments~\cite{iot19}) and provide simple userspace interfaces. \textmu Tiles should be implemented without extensive changes to the Linux and not depend on a specific programming language, so existing applications can be ported easily.\\
\textbf{Efficiency:} \textmu Tiles should be lightweight enough even for embedded devices running on a few megabytes of memory and slow ARM CPUs.\\
\textbf{Performance:} Launching \textmu Tiles, changing their access permissions, sharing across processes, and communications through capability passing should have minimal overhead. Moreover, untrusted (i.e., \textmu Tiles-independent) parts of applications should not suffer any overhead.

To achieve fine-grained isolation with mutual-distrust, we need a security model that lets each thread protect its own \textmu Tiles from untrusted parts of the same thread as well as other threads and processes.
 Simply providing POSIX memory management (e.g. \texttt{malloc} or \texttt{mprotect}) is insufficient. The \textmu Tiles interface needs to ~\rom{1} provide isolation within a single thread;~\rom{2} be flexible for sharing and using \textmu Tiles between threads; and ~\rom{3} provide the capability to restrict unauthorized permission changes or memory mappings modification of allocated \textmu Tiles.

We derive inspiration from Decentralised Information Flow Control (DIFC)~\cite{krohn2007information} but with a more constrained interface -- by not supporting information flow within a program, we avoid the complexities and performance overheads that typically involves.
 Existing DIFC kernels such as HiStar~\cite{zeldovich2006making} achieve our isolation goals, but requires a non-POSIX-based OS that opposes our compatibility goal. To have a practical and lightweight solution, we therefore built \textmu Tiles over a modified Linux kernel, and internally utilizing modern hardware facilities such as ARM memory domains for good performance.





\textbf{Access Control Mechanism}\\
A \textmu Tile is a contiguous allocation of memory that (by default) only its owner thread can access, add/remove pages to/from it, and change its access permission. Our modified Linux kernel enforces the access control via a dynamic security policy based on DIFC~\cite{zeldovich2006making, wang2015between} and a simpler version of the Flume~\cite{krohn2007information} labeling model.

Each thread uses unique tags to denote secrecy or integrity property on its \textmu Tiles. A thread is tagged once it owns at least one \textmu Tile. Each \textmu Tile thread $t$ has one label ${L_{t}}$ that is the set of its unique tags.
Privileges are represented in forms of two capabilities $\theta^{+}$  and $\theta^{-}$ per tag $\theta$ for adding or removing tags to/from labels. These capabilities are stored in a capability list $C_{p}$ per thread $p$.

When thread $p$ owns the $\theta^{+}$ capability ($\theta^{+} \in {C_{p}^{+}}$), it can add $\theta$ to its label ${L_{p}}$, so it gains the privilege to only access \textmu Tile $\theta$ with the default permission set by its owner. Having a $\theta^{-}$ capability lets it remove $\theta$ from its label or declassify \textmu Tile$\theta$. This allows it to change the \textmu Tile's permissions or add/remove pages to it.

The kernel allows information flow from $\alpha$ to $\beta$ only if $L_{\alpha}\subseteq L_{\beta}$. Both $\alpha$ or $\beta$ may use their capabilities to declassify or add a label that could make a flow feasible.
Every thread $p$ may change its label from $L_{i}$ to $L_{j}$ if it has the capability to add tags present in $L_{j}$ but not in $L_{i}$, and can drop the tags that are in $L_{i}$ but not in $L_{j}$. This is formally declared as ($L_{j}-L_{i}\subseteq C_{p}^{+}) \land (L_{i}-L_{j}\subseteq C_{p}^{-} )$.

\textbf{\textmu Tiles Memory Management}\\


To provide in-process isolation (\cref{dp}) and hide the intricacies of hardware domains (\cref{challenges}), we extend the kernel virtual memory management for \textmu Tiles-aware memory mappings, protection, page faults handling, and least privilege enforcement. Then we provide a userspace library on top of our modified kernel, using our \textmu Tiles-specific system calls, for managing \textmu Tiles memory. Example code~\ref{api} shows a basic way of using \textmu Tiles to protect sensitive content in a single thread. 

An application creates a new \textmu Tile by calling \texttt{utile\_create}; the kernel creates a unique tag with both capabilities (since it is the owner) and adds it to the thread's label and capability lists, and returns a unique ID.
Then the owner thread maps pages to its \textmu Tile by calling \texttt{utile\_mmap} that updates the \textmu Tile's metadata with its address space ranges. The kernel allows mappings based on the thread's labels and free hardware domains. If there is a free hardware domain, it maps pages to that domain and places it to \textmu Tiles cache. When the \textmu Tiles already exists in the cache, further access to it is fast. When there is no free hardware domain, we have to evict one of the \textmu Tiles from the cache and map the new \textmu Tile metadata to the freed hardware domain; this requires storing all the necessary information for restoring the evicted \textmu Tile, such as its permission, address space range, and tag. The caching process can be optimized by tuning the eviction rate and suitable caching policies~\cite{park2018libmpk}.

   \begin{table}[t]
\resizebox{\columnwidth}{!}{%

    \begin{tabular}{|l|l|}
    \hline
     Name    & Description                                 \\ \hline
    utile\_create    & Create a new \textmu Tile                       \\ \hline
    utile\_kill    & Destroy a \textmu Tile                       \\ \hline
    utile\_malloc    & Allocate memory within a \textmu Tile                       \\ \hline
    utile\_free     & Deallocate memory from a  \textmu Tile                        \\ \hline
    utile\_mprotect & change an \textmu Tile's pages permission      \\ \hline
    utile\_mmap & Map a page group to a \textmu Tile      \\ \hline
    utile\_munmap & Unmap all pages of a \textmu Tile     \\ \hline
    utile\_get      & Get a \textmu Tile permission      \\ \hline
    \end{tabular}}
    \caption{Userspace \textmu Tile memory management API}
    \label{umem}
\end{table} 



The application uses \texttt{utile\_malloc} and the \textmu Tile ID to allocate memory within the \textmu Tile boundaries (utile\_malloc), and \texttt{utile\_free} to deallocate memory  or \texttt{utile\_mprotect} to change its permissions  (see Table~\ref{umem}). The owner thread can use \texttt{utile\_lock} to restrict unauthorized access to it by accident or other malicious code; this is helpful for in-process attacks inside a single thread. Then application developer can allow only his trusted functions or necessary parts of the code to gain access by calling \texttt{utile\_unlock} (e.g., our single-threaded OpenSSL use case in~\cref{openssl}). 

\input{code.tex}

Our first implementation of \textmu Tiles utilizes ARM memory domains for efficient in-process memory protection; as a result, any code running in supervisor mode can change a domain's access control via the DACR register (\S\ref{memdomain}) or remap private addresses to another domain through the TTBR domain bits. The kernel checks the MMU notifier's callback when unexpected changes are made to TTBR registers but does not directly monitor DACR changes due to the large overhead. Instead, our API and mappings prevent unauthorized permission changes for \textmu Tiles, and we also do not provide a userspace API for direct modification of the DACR.
The security policy enforcement is done by adding custom security hooks in the kernel's virtual memory management system. It checks access based on the correct flow of threads labels (\S\ref{labeling}).
We extend the kernel page fault handler for \textmu Tiles-specific cases. Illegal access to \textmu Tiles causes domain faults which our handler logs (e.g., violating thread information) and terminates it with a signal.




==> mc-api.tex <==
   \begin{table}[htp]
\resizebox{\columnwidth}{!}{%

    \begin{tabular}{|l|l|}
    \hline
     Name    & Description                                 \\ \hline
    imc\_create(hw-mode-flags)$\to{id}$    & Create a new IMC                      \\ \hline
    vdom\_create()$\to{vid}$    & Create a new vdom                      \\ \hline
    imc\_grant($id$,$vid,perms$)    & Grants vdom access permission for an IMC                  \\ \hline
    imc\_revoke($id,vid,perms$)    & Revoke vdom access permission from an IMC                   \\ \hline
    vdom\_malloc($vid,size$)$\to{void*}$    & Allocate memory within an vdom                       \\ \hline
    vdom\_free($vid,void*$)     & Deallocate memory from a  vdom                        \\ \hline
    vdom\_mprotect($vid,...$) & change vdom's pages permission      \\ \hline
    vdom\_mmap($vid,...$)$\to{void*}$ & Map a page group to a vdom      \\ \hline
    vdom\_munmap($vid,...$) & Unmap all pages of a vdom     \\ \hline
    imc\_kill($id$)    & Destroy an IMC                      \\ \hline

    \end{tabular}}
    \caption{Common MCA API.}
    \label{umem}
\end{table} 


==> overview-copy.tex <==
\section{UStar Overview}\label{over}


\begin{figure}[t]
    \includegraphics[width=\columnwidth,height=.25\textheight]{images/ustar.pdf}
    \caption{High-level architecture of uStar; each thread has its label and can tag its own objects so other threads can not access them without having the right label.}
    \label{fig:arch}
\end{figure}

\subsection{Goals and Design}

UStar is a DIFC-based isolation scheme within the Linux kernel that provides thread-granularity privilege separation on ARM architecture with minimal memory footprint. 
The uStar kernel governs information flows through all standard kernel interfaces, including through devices, files, pipes, sockets, and address spaces. DIFC rules are enforced by the kernel on all threads, whether the threads are of the same or different processes. By default resources and threads without an explicit label have empty secrecy and integrity labels, facilitating incremental adoption. In summary, uStar follows the following design goals.

\begin{itemize}
    \item  {\textbf{G1: Fine-grained two-way isolation} uStar needs to strictly restrict any unauthorized access to labeled threads' resources even against compromised root processes.}
    
     \item {\textbf{G2: Compatibility} It is nearly impossible to provide strong security guarantees with no modification or dependency to underlying software or hardware stack and uStar is no exception. However, our system should be compatible with Linux-based kernels, the most used kernel in IoT and mobile industry. It should be implemented without an extensive change of kernel structure, so regular applications do not need any modification.}
     
     \item {\textbf{G3: Minimal memory footprint} our system should be practical and lightweight enough even for IoT devices with only a few Megabytes of memory. }
     
    \item{\textbf{G4: Performance} our solution should incur negligible performance overhead when properly applied. Particularly, running threads within protected domains and changing protected memory access permissions should have no or minimal overhead.
Moreover, isolated components inside a process are often tightly coupled and require cross-domain communications through efficient capability passing and domain switches.}
\end{itemize}

To achieve fine-grained isolation (G1) while minimizing OS incompatibility(G2), uStar extends Linux kernel to enforce DIFC on security-sensitive kernel objects including threads, address spaces, files, or sockets as explained in Section~\ref{objs}. 

Figure~\ref{fig:arch} demonstrates a simplified architecture of uStar's protection levels. UStar-assisted sandbox is only one example of administrative processes running with root privilege. In Android or IoT environment, this is usually done by an application manager that restricts access to sensitive resources based on the application manifest file.
For instance, the sandbox runs as a multi-threaded process that launches applications after isolating sensitive systems resources such as device drivers, file systems, not-allowed sockets, or sensitive config files. Each thread requires its own isolation guarantees in the same address space such as having private memory for storing authentication credentials or stored files in shared file systems (e.g., /tmp/). 

Other applications can benefit from these compartmentalization features as well as the ability to protect their own private resources from privileged processes such as the sandbox itself. As mentioned earlier, there is no concept of super-user in uStar. For example, Figure~\ref{fig:arch} shows how any flow between the sandbox and application's private resources is restricted since they have fully disjoint labels. Figure~\ref{fig:arch} shows a very simplified labeling model for enforcing isolation; detail on uStar labeling is explained in Section ~\ref{labeling}. All of the uStar features are exposed to processes through a simple userspace API (see Table~/ref{syscalls}). 
    



\subsection{Threat Model \& Assumptions}
To achieve G1, we seek to protect each thread's tagged objects against unauthorized, accidental, and malicious data access or disclosure. Our system should protect sensitive kernel and system resources that are labeled during the initialization phase against malicious applications while protecting applications' private resources from privileged system services. This requires the correct implementation and verifiability of DIFC enforcement within the kernel as well as userspace API; it also assumes developers correctly specify their policies through DIFC userspace API for labeling their objects and transferring capabilities.

Hence, uStar's TCB consists of the OS kernel where DIFC enforcement on core kernel objects is implemented.\\
 UStar also depends on ARM memory domains for in-process memory protection, as a result, any code running in supervisor mode can change domains access control through setting DACR register or remap private addresses to another domain through TTBR domain bits[8:5]. UStar checks MMU notifier's callback when unexpected changes are made to TTBR registers. However, protecting DACR is harder since any thread has the right to change its assigned domains' permission and tracking the unauthorized changes will cause large overhead.

UStar does not prevent covert channels based on shared hardware resources(e.g., a hardware cache). Defending against such channels are particularly hard to prevent in DIFC OSes in general. UStar can be completed by Nickel~\cite{sigurbjarnarson2018nickel} framework or hardware-assisted platforms such as Hyperflow~\cite{ferraiuolo2018hyperflow} for side-channel protection on DIFC systems.

 

\subsection{Abstractions \& Labeling in uStar}\label{labeling}

In uStar, programmers use unique tags to denote secrecy or integrity property, but a tag has no inherent meaning; information flow restrictions are enforced only based on the status of labels that are set of tags. Each uStar thread $t$ has two labels, ${S_{t}}$ for secrecy and ${I_{t}}$ for integrity. Each tag is associated with one of these labels and not both to avoid combining two different policy patterns.
For example, as Figure~\ref{fig:arch} shows, an application might create one secrecy tag for its memory block $u$ to store its credentials, and a separate integrity tag for its certificate file $a$, signed by Microsoft. The secrecy tag on the memory block will prevent any unauthorized access or information leak. The integrity tag on file $a$ will prevent a malicious thread from unauthorized modification of the trusted certificate.\\

To be more clear, assigning tags to labels changes the forms of secrecy or integrity lattice~\cite{denning1976lattice} per object.
Assume the bottom of the secrecy lattice is the least restricted label that is public to any principal. The bottom of the integrity lattice is the most trusted label by all principals. Adding secrecy tags to a label restricts the use of the data, moving higher in the lattice. Hence, the most restricted data at the top of the secrecy lattice includes all possible secrecy tags. The bottom of the integrity lattice is the most trusted and includes all integrity tags (endorsed by other principals). Removing integrity tags moves the label higher in the lattice and makes the data less trusted. The top of the integrity lattice has no integrity tags that means no principal endorses it. 

As a result, privileges are represented in forms of two capabilities $\theta^{+}$  and $\theta^{-}$ per tag $\theta$ for adding or removing tags to/from labels. These capabilities are stored in a capability list $C_{p}$ per thread $p$. In terms of secrecy, when thread $p$ owns the $\theta^{+}$ capability ($\theta^{+} \in {C_{p}^{+}}$), it can add $\theta$ to its secrecy label ${S_{p}}$ so it gains the privilege to only receive secret $\theta$ data; and having $\theta^{-}$ capability lets it to remove $\theta$ from its label or declassify any secret $\theta$ data it has seen.\\
In terms of integrity, $\theta^{-} \in {C_{p}^{-}}$ allows the thread to modify $\theta$ data and make it less trusted, while $\theta^{+}$ lets it endorse the current state of $\theta$ as high-integrity and trusted. By default, only objects' owner has both capabilities; uStar provides API for passing capabilities to other threads. In Section~\ref{uapi}, we discuss some of the challenges for efficient and secure transfer of capabilities, in particular between parent and child threads.

Similar to Flume, uStar allows secrecy information flow from $\alpha$ to $\beta$, only if: $S_{\alpha}\subseteq S_{\beta}$. Both $\alpha$ or $\beta$ may use their capabilities to explicitly declassify or add a label that could make a flow feasible. Just like the secrecy rule, uStar allows integrity information flow from $\alpha$ to $\beta$ if: $I_{\beta}\subseteq I_{\alpha}$.\\
In uStar, a thread $p$ may change its label from $L_{i}$ to $L_{j}$ if it has the capability to add tags present in $L_{j}$ but not in $L_{i}$, and can drop the tags that are in $L_{i}$ but not in $L_{j}$. This is formally declared as:\\($L_{j}-L_{i}\subseteq C_{p}^{+}) \land (L_{i}-L_{j}\subseteq C_{p}^{-} )$

\subsection{UStar Objects}\label{objs}

\begin{table}[t]
\resizebox{\columnwidth}{!}{%

    \begin{tabular}{|l|l|}
    \hline
    uStar syscalls                        & Description                                                                                                \\ \hline
    sys\_alloc\_tag                     & Allocate a unique tag                                                                                    \\ \hline
    sys\_modify\_label                    & Modifying or adding new label                                                                              \\ \hline
    sys\_permanent\_declassify            & Permanent declassification                                                                                 \\ \hline
    sys\_temporarily\_declassify          & Temporarily declassification                                                   \\ \hline
    sys\_restore\_capabilities & \makecell{Restoring suspended\\ capabilities}    \\ \hline
    sys\_set\_label\_file              & \makecell{Setting labels to files\\(similar for other objs)} \\ \hline
    sys\_transfer\_capabilities           & \makecell{Passing capabilities to other\\ thread/processes}                                                             \\ \hline
    sys\_label\_udom           & \makecell{Labeling a uStar domain }                                                  \\ \hline
    sys\_enter\_udom             & Entering to protected region                                                                               \\ \hline
    sys\_exit\_udom              & Exiting from protected region                                                                              \\ \hline
    \end{tabular}}
    
\caption{uStar's key system calls}  
\label{syscalls}
\end{table}


Similar to HiStar, uStar's key kernel objects have a secrecy and integrity label. Unlike HiStar's custom kernel, Linux kernel already has fairly complicated layers of abstraction that makes efficient and secure DIFC enforcement challenging; it requires object-specific design principles, interfaces, and user space API (See Tabel~\ref{syscalls}) that we discuss here.\\

\subsubsection{Threads}
    Every thread has a list of secrecy and integrity labels, capabilities, and suspended capabilities. A thread is considered labeled when at least one of the label lists is not empty. Based on the thread's label and capability list, uStar enforces DIFC-based access control on every tagged kernel object by allocating custom hooks in critical kernel points right before accessing the kernel objects.\\
Every thread can create a tag by calling "sys\_alloc\_tag", then, the kernel security module will create and return a new, unique tag. The thread that allocates a tag becomes the owner of the new tag and can give the plus and minus capabilities for the new tag to any other thread.\\
Each thread can specify its security policies by modifying its labels using "sys\_modify\_label" system call. Any thread can declassify its own private objects permanently (sys\_permanent\_declassify) or temporarily (sys\_temporarily\_declassify).\\ 
In particular, temporarily declassification is useful for an efficient share of capabilities between parents and children. For instance, instead of using the API several times for transferring capabilities, the more efficient and secure way is to let child threads inherited only the allowed capabilities by temporarily dropping disallowed capabilities right before creating the child. This way, after clone, the parent can restore the suspended capabilities by calling "sys\_restore\_capabilities".\\
    
 
    
    
\subsubsection{Address Spaces}

\begin{table}
\resizebox{\columnwidth}{!}{%

    \begin{tabular}{|l|l|l|}
    \hline
     Name    & Description                                & Cycles \\ \hline
    udom\_malloc    & Allocate a new ustar domain                & ~      \\ \hline
    udom\_free     & Deallocate a ustar domain                  & ~      \\ \hline
    udom\_mprotect & Set a ustar domain to pages & ~      \\ \hline
    udom\_mmap & Map a page group to a ustar domain & ~      \\ \hline
    udom\_munmap & Unmap all pages of a ustar domain & ~      \\ \hline

    udom\_get      & Get a ustar domain's access right     & ~      \\ \hline
    udom\_set      & Set a ustar domain's access right     & ~      \\ \hline
    get\_domain      & Get a domain's access right     & ~      \\ \hline
    modify\_domain      & Modify a domain access right     & ~      \\ \hline
    \end{tabular}}
    \caption{Overhead of uStar system calls for utilizing and virtualizing ARM memory domains(\textbf{udom} indicates uStar domain) vs standard Linux internal API. The results are averaged of 10 runs of microbenchmarks, where each one executes individual system calI 10 million times while measuring the latency with the PMCCNTR register.}
    \label{udom}
\end{table}

HiStar depends on its custom non-UNIX based kernel for labeling address spaces as a major kernel object. However, labeling address spaces on ARM platforms without extensive change of the Linux kernel structure and adding a large performance overhead was one of the main challenges in building uStar. Any MMU-based permission modifications affect the TLB and userspace cache that causes a large overhead (e.g., due to TLB flushes).\\
As explained in Section~\ref{memdomain}, uStar utilizes ARM memory domains for this purpose. Every thread can assign specific address spaces to one or a few domains (at most 16 domains simultaneously) using "sys\_assign\_label\_domain" system call.\\For each domain, like other kernel objects, there is a kernel data structure for storing labels that are used by uStar for enforcing DIFC checking. Depends on use cases, there are two ways in uStar for changing domains access controls (through setting DACR register) based on DIFC policies. 

\textbf{Channelnges of utilizing ARM memory domains:}\\

\begin{itemize}
\item{Access permissions are inflexible, no readonly by default for example.}
\item{Semantic differences,To change the permission of any page group, MPK modifies
the value of the PKRU. However, the value is effective only in
a single thread because PKRU is thread-local intrinsically as a
register. As a result, different threads in a process can have different permissions for the same page group. This thread-local
inherence helps to improve security for the applications that
require isolation on memory access among different threads,
but hinders MPK from optimizing and improving mprotect().
mprotect() semantically guarantees that page permissions
are synchronized among all threads in a process on which
particular applications rely. This not only makes it difficult to
accelerate mprotect() with MPK, but also breaks the guarantee of execute-only memory implemented on mprotect in the
latest kernel. mprotect() supporting executable-only memory
relying on MPK does not consider synchronization among
threads, which developers basically expect of mprotect().
Even when the kernel successfully allocates a key for the
execute-only page, another thread might have a read access to
it due to a lack of synchronization. To make MPK a drop-in
replacement of mprotect() for both security and usability,
developers need to synchronize the PKRU values among all the
threads.}
    \item {Potential Security Problem on fixed number of domains, it reducese the security risks if developer doens't know the number of domains}
    \item{Currently, ARM relies on a 32-bit DACR such that it supports
up to 16 keys. Developers are responsible for ensuring that
an application never creates more than 16 page groups at the
same time. This implies that developers have to examine at
runtime the number of active page groups, which are used
by both the application itself and the third-party libraries it
depends on. Otherwise, the program may fail to properly benefit from MPK. This issue undermines the usability of MPK
and discourages developers from utilizing it actively. Using
a large register (e.g., 1024 bits) does not scale because MPK
needs additional storage to associate keys with pages. For
example, to support 512 protection keys, nine bits are necessary for each PTE, requiring enlarged page tables, shrunken
address bits, or separate storage}
\end{itemize}



\textbf{How uStar utilizes domains?}\\

To utilize MPK for domain-based isolation and as a
substitute for mprotect(), we have to overcome the three challenges: (1) insecure key management, (2) hardware resource
limitations, and (3) different semantics from mprotect().
libmpk adopts two approaches: (1) key virtualization, and
(2) inter-thread key synchronization, which effectively solve
the challenges.

ustar enables labeling memory domains by virtualizing ARM memory domains so we can assign unique tags while hardware only supports 16 domains. so applications can add or modify an ddress space labels using sys\_label\_udom. Then applicatiocan use 
udom\_mmap(), to change the permissions of an udom domain. SImilary uStar garantees to allocate and deallocate memory from a udom using  udom\_alloc and udom\_free.

\textbf{udom\_alloc and udom\_free.}\\
\textbf{udom\_get and udom\_set.}\\
\textbf{udom\_mprotect.}\\


\begin{table}[t]
\resizebox{.6\columnwidth}{!}{%

    \begin{tabular}{|l|l|}
    \hline
    Name                     & Latency \\ \hline
    udom\_alloc    & ~       \\ \hline
    malloc                   & ~       \\ \hline
    udom\_free               & ~       \\ \hline
    free                     & ~       \\ \hline
    udom\_mprotect & ~       \\ \hline
    mprotect                 & ~       \\ \hline
    \end{tabular}}
    \caption{comparison of uStar base memory operations vs standard Linux}
\end{table}

   \begin{itemize} 
       
  \item \textbf{Lazy DIFC checking}\\
    From an application developer perspective, this is the easiest way to ensure DIFC enforcement on already assigned domains without using any API. Since any violation of access controls on domains causes a domain fault, uStar's fault handler first detects which domain is violated and by whom. Then it checks if the access is allowed using a custom hook (security\_difc\_labels\_allowed). It changes domain access mode in case the violated thread has the right capability, otherwise, it kills the malicious thread and does not change the domain mode.\\
    
   \item  \textbf{Secured gates}\\
UStar also provides specific entries for applications to manually specify their active domains and modify their access permissions. Using system call "sys\_ustar\_enter\_domain", labeled-thread specifies its active domains and uStar ensures while it is running in that domain, no other thread can access its contents or change its access mode. Threads can make their domains free by calling "sys\_ustar\_exit\_domain".

   \end{itemize} 


\subsubsection{Files and Directorie}

UStar protects files again any unauthorized file operation including getting stat or listing labeled files or directories by a minimal number of file systems modification. For tagging files and directories, every inode object security feature has a label assigned to it; similar to other objects. Threads can create and modify their files or directories labels using "sys\_set\_label\_file" system call. \\
Since most embedded and Android file systems do not support extended attributes,  uStar is not depended on that for permanently storing labels and adds custom hooks for essential labeling operations such as allocation, storage, and modification. UStar security policies are simple and small enough so they add very small memory overhead at runtime.\\
Unlike Flume or Capsicum, uStar does not extend the file descriptor abstraction that requires extensive modification or restrictions of most file system related system calls. UStar provides file system isolations through enforcing DIFC at the highest level of abstraction mostly in VFS layer and pathname lookup (namei) to minimalize changes for each supported file system. For example, uStar extends VFS operations (adds ~300 LoC) for creating labeled paths and enforcing DIFC permissions. \\
    
    
  \subsubsection{Network sockets and IPC pipes} 

    Labeling inodes associated with other Linux abstractions, such as pipes and sockets, are similar to files. However, enforcing DIFC permissions is done by extending security hooks for socket operations. For example, uStar checks DIFC policies during creation or modification of any socket structure by adding security hooks such as "ustar\_socket\_create" or "ustar\_socket\_post\_create", or before establishing a Unix domain stream connection (ustar\_unix\_stream\_connect).


    


==> utiles_arch.tex <==

\begin{figure*}
\centering
\includegraphics[scale=.42]{images/thrd.pdf}
\caption{\textmu Tiles threading abstraction: each thread is a security principal, it can define security policies for controlling its \textmu Tiles collection, and pass its capabilities to other threads. The kernel enforces the security policies and handles virtual memory management of \textmu Tiles.}
\label{threading}
\end{figure*}
